Extended Version: Multi-Robot Motion Planning with Cooperative Localization

We consider the uncertain multi-robot motion planning (MRMP) problem with cooperative localization (CL-MRMP), under both motion and measurement noise, where each robot can act as a sensor for its nearby teammates. We formalize CL-MRMP as a chance-constrained motion planning problem, and propose a safety-guaranteed algorithm that explicitly accounts for robot-robot correlations. Our approach extends a sampling-based planner to solve CL-MRMP while preserving probabilistic completeness. To improve efficiency, we introduce novel biasing techniques. We evaluate our method across diverse benchmarks, demonstrating its effectiveness in generating motion plans, with significant performance gains from biasing strategies.

==> sections/evaluations.tex <==


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.2\textwidth}
        \centering
        \fontsize{5}{5}\selectfont 
        \includegraphics[width=\textwidth,trim={1.6cm 1.2cm 1.2cm 1.2cm}, clip]{figures/Environments/corridor_trajectory.pdf}
        \caption{\small Corridor}
        \label{fig:Corridor Environemnt}
    \end{subfigure}
    ~~~~~~
    \begin{subfigure}[b]{0.11\textwidth}
        \centering
        \fontsize{5}{5}\selectfont 
        \includegraphics[width=\textwidth,trim={3.9cm 0.7cm 3.7cm 0.7cm}, clip]{figures/Environments/Pincer_labeled.pdf}
        \caption{\small Pincer}
        \label{fig:Pincer Environemnt}
    \end{subfigure}
    \hspace{5mm}
    
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \fontsize{5}{5}\selectfont 
        \includegraphics[width=\textwidth,trim={2.7cm 0.7cm 2.4cm 0.7cm}, clip]{figures/Environments/Hive_labeled.pdf}
        \caption{\small Hive}
        \label{fig:Hive Environemnt}
    \end{subfigure}
    ~~~~
    \begin{subfigure}[b]{0.18\textwidth}
        \centering
        \fontsize{5}{5}\selectfont 
        \includegraphics[width=\textwidth,trim={2.7cm 0.7cm 2.4cm 0.7cm}, clip]{figures/Environments/Random_labeled.pdf}
        \caption{\small Random}
        \label{fig:Random Environemnt}
    \end{subfigure}
    \caption{\small Test Environments}
    \label{fig:envs}
    \vspace{-5mm}
\end{figure}




% \ml{add validation results uing MC simulation. Add an example traj per env?}

% We evaluated our algorithm in four environments: `Corridor', `Hive', `Pincer', and `Random', shown in Fig.~
% \ref{fig:envs}. 
% \ref{fig:Hive Environemnt}, \ref{fig:Pincer Environemnt}, \ref{fig:Random Environemnt} respectively. 
% Robot start locations are indicated by stars, and goal regions by shaded circles labeled by robot index. 
%
% We compare the Belief-$RRT$ and Belief-$EST$ planners, and each of the proposed biasing techniques with biasing rates ($\epsilon$) from $0.01$ to $0.5$, comparing to a baseline with no biasing. Each benchmark contains $50$ runs for each planning instance. We report the success rate as the fraction of successful planning instances as well as boxplots of both the time and number of iterations when solutions are found, as shown in Fig.~\ref{fig:2 Robot Environments}, where all figures use the same legend \qh{a little weird that the results are described in this sentence before the set up}. The planning time is set to $1$ minute for the Hive environment, and $2$ minutes for all others. Benchmarks were performed on an Intel Core i7-12700K CPU and 32GB of RAM.

% We evaluate our algorithm to assess its performance across different environments and biasing techniques. Specifically, we test it in four environments, `Corridor', `Hive', `Pincer', and `Random', as shown in Fig.~\ref{fig:envs}. 
% The goal is to compare the effectiveness of the planners and biasing strategies in solving the CL-MRMP problem.

% We implemented the planners (Belief-RRT and Belief EST) in OMPL \ml{CITE}, and ran benchmarks on an Intel Core i7-12700K CPU with 32GB of RAM. Each environment consists of predefined robot start locations (indicated by stars) and goal regions (shaded circles labeled by robot index). We compare the Belief-$RRT$ and Belief-$EST$ planners, evaluating each proposed biasing technique with biasing rates ($\epsilon$) ranging from $0.01$ to $0.5$, and include a baseline with no biasing. Each benchmark consists of $50$ runs for each planning instance. The planning time is set to $1$ minute for the Hive environment and $2$ minutes for all others.
% 
% To analyze performance, we report the success rate as the fraction of successful planning instances. Additionally, we provide boxplots of both the computation time and the number of iterations required to find a solution.
% , as shown in Fig.~\ref{fig:2 Robot Environments}, where all figures follow the same legend.

We evaluate our algorithm across four environments shown in Fig.~\ref{fig:envs}
to assess performance across different planners and biasing techniques. Robot start locations (stars) and goal regions (shaded circles) are predefined.
We implemented the planners (Belief-RRT and -EST) in OMPL \cite{sucan2012the-open-motion-planning-library} and ran all experiments on an Intel Core i7-12700K CPU with 32GB~RAM. 

% comparing Belief-$RRT$ and Belief-$EST$ planners with biasing rates ($\epsilon$) from $0.01$ to $0.5$, alongside a no-biasing baseline. Each instance is run $50$ times, with a planning time of 1 minute for `Hive' and 2 minutes for others. We report success rates, computation time, and iteration counts, summarized in Fig.~\ref{fig:2 Robot Environments}, where all figures follow the same legend.




In all cases, each robot has 2D dynamics given by: $A_k^i = B_k^i = I_{2\times 2}$, $Q_k^i = 0.01I_{2\times 2}$. A subset of robots (corresponding to odd indices $i$) has access to proprioceptive measurements, making the system unobservable in the absence of exteroceptive measurements. Primary results are reported with two robots, scaling results are reported up to six robots, with additional results in the extended version of this paper \cite{Theurkauf_extended}.
% This mimics a systems where only a few robots have access to high fidelity self-measurements, like GPS, while the other robots must rely on relative measurements like range. 
%In practice this means that the marginal uncertainty of the robots that lack proprioceptive measurements will grow unbounded without access to exteroceptive measurements. 
The %proprioceptive 
measurement model is given by 
$C_k^{i,prop}=I_{2\times 2}$ and %exteroceptive measurements by 
$C_k^{ij,ext}=[I_{2\times 2}, -I_{2\times 2}]$. The chance constraints are set to $p_{obs}=p_{rob}=p_{\neg CL}=0.05$.



% e.g. for a two robot system is modeled as:
% \begin{align}
%     Y_k^{prop} &= \begin{bmatrix}
%         1 & 0 & 0 & 0  \\
%         0 & 1 & 0 & 0
%     \end{bmatrix} \begin{bmatrix}
%     x_k^1 \\
%     x_k^2
%     \end{bmatrix} + V_k^{prop} \\
%     Y_k^{ext} &= \begin{bmatrix}
%         1 & 0 & -1 & 0  \\
%         0 & 1 & 0 & -1
%     \end{bmatrix} \begin{bmatrix}
%     x_k^1 \\
%     x_k^2
%     \end{bmatrix} + V_k^{ext}
% \end{align}

\subsection{Illustrative Examples}
Figs.~\ref{fig:Random trajectory} and~\ref{fig:Corridor Environemnt} show two example trajectories for the Random and Corridor environments, respectively.
% Fig.~\ref{fig:Random trajectory} shows an example trajectory for the Random environment. %is shown in Fig.~\ref{fig:Random trajectory}. 
The cyan robot states are unobservable without CL, as shown in Fig.~\ref{fig:Random trajectory zoom}. %where time is added as the z axis, 
In Fig.~\ref{fig:Random trajectory} the red robot must divert to enable CL so that the cyan robot %can reach it's 
reaches its goal. In Fig.~\ref{fig:Corridor Environemnt}, the cyan robot diverts to remain close to the red robot throughout its trajectory and keep its uncertainty small.
An online method that only drives toward the goal would fail to find these cooperative behaviors, and a decoupled approach that does not account for CL would fail to plan for the %unobservable 
An online method that only drives toward the goal would fail to find these cooperative behaviors, and a decoupled approach that does not account for CL would fail to plan for the %unobservable 
cyan robot. Our algorithm finds both plans within 2 minutes.

% \qh{Somehow need some overall statement on the proposed methods. Like, high success rate across all environments... For all of these problems, the robots are required to CL?}

% where time is added as the z axis, in the first few time steps the uncertainty grows until the second robot (red) is within CL range, then shrinks when CL is enabled. In order for the second robot to reach its goal, the first robot must divert to aid the second. Because the first robot has access to proprioceptive measurements, it can then continuing to its own goal without CL. 

% \begin{figure}
%     \centering
%     \begin{subfigure}[b]{0.26\textwidth}
%         \centering
%         \fontsize{5}{5}\selectfont 
%         \includegraphics[width=\textwidth,trim={3cm 1.2cm 2cm 0.5cm}, clip]{figures/Random Results/random_fulltraj.pdf}
%         \caption{Trajetory}
%         \label{fig:Random trajectory}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.22\textwidth}
%         \centering
%         \fontsize{5}{5}\selectfont 
%         \includegraphics[width=\textwidth,trim={3cm 1cm 3.2cm 1cm}, clip]{figures/Random Results/random_trajzoom2.pdf}
%         \caption{Trajectory zoom with time dimension}
%         \label{fig:Random trajectory zoom}
%     \end{subfigure}
%     \caption{Random Environment, Example Trajectory}
%     \label{fig:example traj}
% \end{figure}



%%%%%%  TWO ROBOT ENVIRONMENTS

% Corridor, Hive, Random: squished
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.9\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/legend_crop.pdf}
    \end{subfigure}
    \newline
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3.2cm}, clip]{figures/ShrinkResults/Corridor Results/corridor_SR.pdf}
        \caption{\small Corridor, Success Rate}
        \label{fig:Corridor success rate}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.7cm 3cm 3.5cm 3.2cm}, clip]{figures/ShrinkResults/Corridor Results/corridor_ST.pdf}
        \caption{\small Corridor, Solution Time}
        \label{fig:Corridor solution time}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/Corridor Results/corridor_SI.pdf}
        \caption{\small Corridor, Number Iterations}
        \label{fig:Corridor number iterations}
    \end{subfigure}
    \newline
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3.2cm}, clip]{figures/ShrinkResults/Hive2 Results/hive2_SR.pdf}
        \caption{\small Hive, Success Rate}
        \label{fig:Hive2 success rate}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.7cm 3cm 3.5cm 3.2cm}, clip]{figures/ShrinkResults/Hive2 Results/hive2_ST.pdf}
        \caption{\small Hive, Solution Time}
        \label{fig:Hive2 solution time}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/Hive2 Results/hive2_SI.pdf}
        \caption{\small Hive, Number Iterations}
        \label{fig:Hive2 number iterations}
    \end{subfigure}
    \newline
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3.2cm}, clip]{figures/ShrinkResults/Random Results/random_SR.pdf}
        \caption{\small Random, Success Rate}
        \label{fig:Random success rate}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.7cm 3cm 3.5cm 3.2cm}, clip]{figures/ShrinkResults/Random Results/random_ST.pdf}
        \caption{\small Random, Solution Time}
        \label{fig:Random solution time}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/Random Results/random_SI.pdf}
        \caption{\small Random, Number Iterations}
        \label{fig:Random number iterations}
    \end{subfigure}
    \caption{\small Two Robot Environments}
    \label{fig:2 Robot Environments}
\end{figure*}



% Hive, Pincer, Corridor, Random
% \begin{figure*}
% \caption{Two Robot Environments}
% \label{fig:2 Robot Environments}
%     \centering
%     \begin{subfigure}[b]{0.9\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/legend_crop.pdf}
%     \end{subfigure}
%     \newline
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Hive2 Results/hive2_SR.pdf}
%         \caption{Hive, Success Rate}
%         \label{fig:Hive2 success rate}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Pincer2 Results/pincer2_SR.pdf}
%         \caption{Pincer, Success Rate}
%         \label{fig:Pincer2 success rate}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Corridor Results/corridor_SR.pdf}
%         \caption{Corridor, Number Iterations}
%         \label{fig:Corridor success rate}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Random Results/random_SR.pdf}
%         \caption{Random, Number Iterations}
%         \label{fig:Random success rate}
%     \end{subfigure}
%     \newline
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Hive2 Results/hive2_ST.pdf}
%         \caption{Hive, Solution Time}
%         \label{fig:Hive2 solution time}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Pincer2 Results/pincer2_ST.pdf}
%         \caption{Pincer, Solution Time}
%         \label{fig:Pincer2 solution time}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Corridor Results/corridor_ST.pdf}
%         \caption{Corridor, Number Iterations}
%         \label{fig:Corridor solution time}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Random Results/random_ST.pdf}
%         \caption{Random, Number Iterations}
%         \label{fig:Random solution time}
%     \end{subfigure}
%     \newline
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Hive2 Results/hive2_SI.pdf}
%         \caption{Hive, Number Iterations}
%         \label{fig:Hive2 number iterations}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Pincer2 Results/pincer2_SI.pdf}
%         \caption{Pincer, Number Iterations}
%         \label{fig:Pincer2 number iterations}
%     \end{subfigure}        
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Corridor Results/corridor_SI.pdf}
%         \caption{Corridor, Number Iterations}
%         \label{fig:Corridor number iterations}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.24\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Random Results/random_SI.pdf}
%         \caption{Random, Number Iterations}
%         \label{fig:Random number iterations}
%     \end{subfigure}
% \end{figure*}



% Corridor, Hive, Random
% \begin{figure*}
% \caption{Two Robot Environments}
% \label{fig:2 Robot Environments}
%     \centering
%     \begin{subfigure}[b]{0.9\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{figures/legend_crop.pdf}
%     \end{subfigure}
%     \newline
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Hive2 Results/hive2_SR.pdf}
%         \caption{Hive, Success Rate}
%         \label{fig:Hive2 success rate}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Corridor Results/corridor_SR.pdf}
%         \caption{Corridor, Number Iterations}
%         \label{fig:Corridor success rate}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Random Results/random_SR.pdf}
%         \caption{Random, Number Iterations}
%         \label{fig:Random success rate}
%     \end{subfigure}
%     \newline
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Hive2 Results/hive2_ST.pdf}
%         \caption{Hive, Solution Time}
%         \label{fig:Hive2 solution time}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Corridor Results/corridor_ST.pdf}
%         \caption{Corridor, Number Iterations}
%         \label{fig:Corridor solution time}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Random Results/random_ST.pdf}
%         \caption{Random, Number Iterations}
%         \label{fig:Random solution time}
%     \end{subfigure}
%     \newline
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Hive2 Results/hive2_SI.pdf}
%         \caption{Hive, Number Iterations}
%         \label{fig:Hive2 number iterations}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Corridor Results/corridor_SI.pdf}
%         \caption{Corridor, Number Iterations}
%         \label{fig:Corridor number iterations}
%     \end{subfigure}
%     \begin{subfigure}[b]{0.32\textwidth}
%         \centering
%         \includegraphics[width=\textwidth,trim={0.8cm 0.2cm 1.5cm 0.7cm}, clip]{figures/Random Results/random_SI.pdf}
%         \caption{Random, Number Iterations}
%         \label{fig:Random number iterations}
%     \end{subfigure}
% \end{figure*}


\subsection{Benchmarks}
We use benchmarks to compare Belief-$RRT$ and Belief-$EST$ planners with biasing rates ($\epsilon$) from $0.01$ to $0.5$, alongside a no-biasing baseline. Each instance is run $50$ times, with a planning time of 1 minute for `Hive' and 2 minutes for others. We report success rates, computation time, and iteration counts, summarized in Figs.~\ref{fig:2 Robot Environments} and~\ref{fig:4}, where all plots follow the same legend.

Overall, the results show that our proposed algorithm reliably finds solutions in each environment with both RRT and EST variants, and biasing techniques better suited to some over others. In particular, we observe that Re-branching can improve planning time and iterations in simple environments, and RRT with Cloning scales well with $N_A$. Detailed discussion is provided below. 

% Overall, the results demonstrate that our proposed algorithm consistently finds solutions across all environments, with different planners (RRT, EST) and biasing techniques performing better in certain scenarios. In particular, we observe that Re-branching improves planning time and iterations in simpler environments, while RRT with Cloning scales well with the number of agents ($N_A$). A detailed discussion of these results is provided below.




\textbf{CL vs. Robot-robot collision: }
%The CL problem is complex, and biasing can have unpredictable results. Exploration of state where robots are close together necessarily conflicts with safety (robot-robot collision). 
To illustrate the tension introduced between CL and robot-robot collisions, %this, 
consider the boxplots of the proportion of nodes rejected for robot-obstacle collision (Fig.~\ref{fig:Random obs coll}) and robot-robot collision (Fig.~\ref{fig:Random robot coll}) for the Random environment. %Observe that, 
As $\epsilon$ increases, %the %biasing rate increases, 
%the 
robots are drawn closer together, causing more robot-robot collisions. This is particularly true of %the 
Re-branching, %technique, 
indicating that (despite the high computation cost) it is the most effective CL biasing method. %for bringing robots closer together. 
We can see further evidence of this in the simpler 2-robot Hive environment, %which is simple enough to 
where the small search space is more tolerant of %which overcomes 
Re-branching's cost. 
%inefficiencies of Re-branching.
\begin{figure*}
    \centering
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/Random Results/random_obscol.pdf}
        \caption{\small Random, Robot-Obstacle Collision Rate}
        \label{fig:Random obs coll}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \centering
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/Random Results/random_robcol.pdf}
        \caption{\small Random, Robot-Robot Collision Rate}
        \label{fig:Random robot coll}
    \end{subfigure}
    \begin{subfigure}[b]{0.32\textwidth}
        \includegraphics[width=\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/PincerRRT Results/pincer_RRTclone_SR.pdf}
        \caption{\small Pincer, RRT Cloning Method}
        \label{fig:Pincer RRT clone}
    \end{subfigure}
    \caption{\small Benchmarking results for (a)-(b) collision rates of 2 robots in Random Env., and (c) success rates for 2-6 robots in Pincer Env.}
    \label{fig:4}
    \vspace{-2mm}
\end{figure*}

\textbf{Re-branching:} 
Re-branching is an effective biasing technique in that it can efficiently find a solution for simple cases.
% , as seen in the two robot Hive environment shown in Fig.~\ref{fig:2 Robot Environments}. 
In particular, re-branching shows a substantial decrease in solution times (Fig.~ \ref{fig:Hive2 solution time}) and number of iterations (Fig.~\ref{fig:Hive2 number iterations}) from the baseline compared to all other techniques for the same success rate (Fig.~\ref{fig:Hive2 success rate}). However, because Re-branching is computationally intensive its performance can drop rapidly as more robots are added or for complex environments. This indicates that a more efficient re-branching method could be a promising future direction. 
% We leave this to future work.

\textbf{Cloning:} 
RRT with Cloning performs well in the Pincer environment for larger $N_A$, increasing the success rate from $0.86$ to $0.68$ for four robots, and $0.04$ to $0.5$ for five robots (Fig.~\ref{fig:Pincer RRT clone}). 
% Also note that while EST generally does worse than RRT in the Pincer environment, for the three robot case EST with Cloning increases the success from from $0.76$ to $0.98$ while significantly decreasing the solution time and number of robots, as seen in Fig.~\ref{fig:Pincer3 Results} in the Appendix. 
This indicates that the simplicity of the Cloning method can be quite effective for larger robot teams.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.32\textwidth,trim={2.8cm 3cm 3.5cm 3cm}, clip]{figures/ShrinkResults/PincerRRT Results/pincer_RRTclone_SR.pdf}
%     \caption{Pincer Environment, RRT Cloning Method}
%     \label{fig:Pincer RRT clone}
% \end{figure}

\textbf{Distance Weighting:}
The Distance Weighting technique has the most ambiguous effect on performance, with no obvious advantages anywhere in Fig.~\ref{fig:2 Robot Environments}.
% \qh{Can you show where on the figures?}\at{Difficult, its more that it is never the best method across the board}. 
The increased computation of Weighting likely outweighs any benefits of the biasing technique, especially with larger $N_A$.
% (this can be seen in the high computation times of Weighting vs Cloning especially in Fig.~\ref{fig:Pincer3 Results}
A simpler method of calculating the weights may improve results. See the extended version of this paper for further discussion \cite{Theurkauf_extended}.

% \at{This one is not great, can cut it??? I like it though....}
% \nra{if room, can briefly mention that this was examined and quickly summarize main findings, without having to fully report on it}
% \ml{I agree with Anne.  We don't learn anything from it.  Let's remove it?}
% The Distance Weighting technique has the most ambiguous effect on performance: it generally either has negligible or deleterious effect on the success rate, with similarly unimpressive results in solution and number of iterations. However, in the Random environment it seems to provide modest improvement in success rate, and does at least as well as Cloning, see Figs.~\ref{fig:Random success rate}, \ref{fig:Random solution time}, \ref{fig:Random number iterations}. 
% % It has a similar effect for three and four robots in the Hive environment, see Figs.~\ref{fig:Hive3 Results} and \ref{fig:Hive4 Results} respectively in the Appendix.

% This underperformance is unintuitive: Distance Weighting directly reasons over the distances between robots within a node, rather than indirectly biasing like the Cloning technique. It is possible that the increased computation of Weighting outweighs any benefits of the biasing technique, especially with larger numbers of robots
% % (this can be seen in the high computation times of Weighting vs Cloning especially in Fig.~\ref{fig:Pincer3 Results}
% . A simpler method of calculating the weights may improve results.

\textbf{Planner Type: }
Finally, note that EST generally performs better in the Random and Hive environments, while RRT performs better in the Pincer environment. Both perform similarly well in the Corridor environment. This possibly due to the topology of the environments. RRT tends to pull tree growth to unexplored parts of the state space (via Voronoi biasing), while EST more exhaustively explores the space outward from the initial (via sparsity). In the Pincer environemnt RRT more successfully pulls the search tree through the passage and explores the goal side, whereas EST is slow to explore the entire space. On the other hand, the Hive and Random environments do not require extensive searches (especially the Hive), and therefore the exhaustive EST search more quickly finds satisfying plans. The Corridor environment is not particularly suited to either method of tree expansion.
